NeVAE: A Deep Generative Model for Molecular Graphs

Deep generative models have been praised for their ability to learn smooth latent representation of images, text, and audio, which can then be used to generate new, plausible data. However, current generative models are unable to work with molecular graphs due to their unique characteristics-their underlying structure is not Euclidean or grid-like, they remain isomorphic under permutation of the nodes labels, and they come with a different number of nodes and edges. In this paper, we first propose a novel variational autoencoder for molecular graphs, whose encoder and decoder are specially designed to account for the above properties by means of several technical innovations. Moreover, in contrast with the state of the art, our decoder is able to provide the spatial coordinates of the atoms of the molecules it generates. Then, we develop a gradient-based algorithm to optimize the decoder of our model so that it learns to generate molecules that maximize the value of certain property of interest and, given a molecule of interest, it is able to optimize the spatial configuration of its atoms for greater stability. Experiments reveal that our variational autoencoder can discover plausible, diverse and novel molecules more effectively than several state of the art models. Moreover, for several properties of interest, our optimized decoder is able to identify molecules with property values 121% higher than those identified by several state of the art methods based on Bayesian optimization and reinforcement learning

==> 060related.tex <==
Our model is conceptually related to previous work on random graph models, network representation learning and
recent advances in variational autoencoders and their applications to complex data.

\xhdr{Random graph models} Since the seminal random graph model by Erdos-R{\'e}nyi~\cite{erdos1960evolution}, where each pair of nodes is connected by an edge with 
probability $p$, there is a long history of random graph models in the literature~\cite{watts1998collective, waxman1988routing, barabasi1999emergence,  karrer2011stochastic, leskovec2005graphs, leskovec2010kronecker, holland1981exponential}.
%
Most of these random graph models aim to generate graphs that match one or more properties observed in of real-world graphs, \eg, heavy-tailed node degree distributions~\cite{barabasi1999emergence, karrer2011stochastic}, 
small diameter~\cite{watts1998collective, waxman1988routing}, or densification power-law~\cite{leskovec2005graphs, leskovec2010kronecker}.
%
However, most of the above random graph models share one or more of the following limitations: (i) they make strong (parametric) assumptions about the underlying generative process of the graphs they model; 
(ii) their parameters are difficult to learn from real-world graph data; and, (iii) they have a limited expressive power and are unable to generate diverse set of graphs.
%
Only very recently, there have been a paucity of work on deep generative model for graphs~\cite{welling, graphgan, graphvae, iclr2018graphs}. Among them, the most closely related works~\cite{welling, graphvae}, which also propose variational autoencoders for graphs, are not invariant to permutation of the node labels, cannot generate (or be trained with) graphs with different number of nodes nor guarantee a set of local structural and functional properties in the generated graphs.
%

%
\xhdr{Network representation learning} In recent years, there has been a flurry of research that seeks to learn low dimensional re\-pre\-sen\-ta\-tions---embeddings---that 
encode the structural information about a graph. These embeddings can be then used as input features for several downstream machine learning tasks such as link prediction 
or node classification. 
%
Most of the approaches in the literature are based on matrix factorization~\cite{belkin2002laplacian, ahmed2013distributed, cao2015grarep}, random walks~\cite{grover2016node2vec, perozzi2014deepwalk},
or neighborhood aggregation functions~\cite{hamilton2017inductive}, which include graph convolution networks (GCNs)~\cite{kipf2016semi, schlichtkrull2017modeling, berg2017graph, li2018adaptive, zhang2018end}.
%
Hamilton et al.~\cite{hamilton2017representation} provides a comprehensive survey.
%
However, this line of work is orthogonal to our work since it does not provide a random graph model to generate new, plausible graphs as we do.

%
\xhdr{Variational autoencoders (VAEs)} The framework of variational autoencoders has emerged as a powerful technique to design complex, 
data-driven nonlinear generative models that are able to generate new plausible data.
%
However, VAEs for graphs are still in their infancy~\cite{welling, graphvae}, as discussed above. Currently, VAEs have been mostly designed for image, audio 
and text generation~\cite{bowman2015generating, hu2017toward, yang2017improved, radford2015unsupervised}.
%
Very recently, the development of VAEs for text generation with a grammar~\cite{gomez2016automatic,olivecrona2017molecular,kusner2017grammar} have 
facilitated their use in molecule discovery. However, such models use a string representations of molecules (\eg, SMILES) and, as a consequence, are more 
prone to generating invalid molecules than our variational autoencoder for graphs.
%
